Relational Graph Transformer

Relational Deep Learning (RDL) is a promising approach for building state-of-the-art predictive models on multi-table relational data by representing it as a heterogeneous temporal graph. However, commonly used Graph Neural Network models suffer from fundamental limitations in capturing complex structural patterns and long-range dependencies that are inherent in relational data. While Graph Transformers have emerged as powerful alternatives to GNNs on general graphs, applying them to relational entity graphs presents unique challenges: (i) Traditional positional encodings fail to generalize to massive, heterogeneous graphs; (ii) existing architectures cannot model the temporal dynamics and schema constraints of relational data; (iii) existing tokenization schemes lose critical structural information. Here we introduce the Relational Graph Transformer (RelGT), the first graph transformer architecture designed specifically for relational tables. RelGT employs a novel multi-element tokenization strategy that decomposes each node into five components (features, type, hop distance, time, and local structure), enabling efficient encoding of heterogeneity, temporality, and topology without expensive precomputation. Our architecture combines local attention over sampled subgraphs with global attention to learnable centroids, incorporating both local and database-wide representations. Across 21 tasks from the RelBench benchmark, RelGT consistently matches or outperforms GNN baselines by up to 18%, establishing Graph Transformers as a powerful architecture for Relational Deep Learning.

==> minipage_format.tex <==
\begin{table}[ht]
\centering
\begin{minipage}{.49\textwidth}
\centering
\small
\caption{Results on the entity classification tasks in RelBench. Higher is better. Best values are in \textbf{bold}. Relative gains are in percentage.}
\label{tab:main-results-classification}
\scalebox{0.63}{
\begin{tabular}{llccccc}
\toprule
\textbf{Dataset} & \textbf{Task (\# train)} & \textbf{AUC $\uparrow$} & \makecell{\textbf{RDL}\\\textbf{Baseline}} & \makecell{\textbf{Rel-GT}\\ \textbf{(ours)}} & \makecell{\textbf{Rel.}\\ \textbf{Gain}} \\
\midrule

\multirow{4}{*}{rel-f1} 
 & \multirow{2}{*}{driver-dnf (11k)} & Test & 0.7262 & \textbf{0.759} & 4.52 \\
 & & Val & 0.7136 & 0.680 &  \\
 & \multirow{2}{*}{driver-top3 (1k)} & Test & 0.7554 & \textbf{0.835} & 10.54 \\
 & & Val & 0.7764 & 0.796 & \\
\midrule
\multirow{4}{*}{rel-avito}
 & \multirow{2}{*}{user-clicks (59k)} & Test & 0.6590 & \textbf{0.683} & 3.64 \\
 & & Val & 0.6473 & 0.665 &  \\
 & \multirow{2}{*}{user-visits (86k)} & Test & 0.6620 & \textbf{0.668} & 0.91 \\
 & & Val & 0.6965 & 0.702 & \\

\midrule
\multirow{4}{*}{rel-event}
 & \multirow{2}{*}{user-repeat (3k)} & Test & \textbf{0.7689} & 0.756 & -1.68 \\
 & & Val & 0.7125 & 0.725 &  \\
 & \multirow{2}{*}{user-ignore (19k)} & Test & \textbf{0.8162} & \textbf{0.816} & 0.00 \\
 & & Val & 0.9170 & 0.887 &  \\

\midrule
\multirow{2}{*}{rel-trial}
 & \multirow{2}{*}{study-outcome (11k)} & Test & \textbf{0.6860} & \textbf{0.686} & 0.00 \\
 & & Val & 0.6818 & 0.668 &  \\

 \midrule
\multirow{4}{*}{rel-amazon}
 & \multirow{2}{*}{user-churn (4.7m)} & Test & 0.7042 & \textbf{0.705} & 0.11 \\
 & & Val & 0.7045 & 0.706 &  \\
 & \multirow{2}{*}{item-churn (2.6m)} & Test & \textbf{0.8281} & 0.826 & -0.25\\
 & & Val & 0.8239 & 0.822 &  \\

 \midrule
\multirow{4}{*}{rel-stack}
 & \multirow{2}{*}{user-engagement (1.4m)} & Test & 0.9021 & \textbf{0.906} & 0.43 \\
 & & Val & 0.9059 & 0.904 &  \\
 & \multirow{2}{*}{user-badge (3.4m)} & Test & \textbf{0.8986} & 0.863 & -3.96 \\
 & & Val & 0.8886 & 0.874 &  \\

\midrule
\multirow{2}{*}{rel-hm}
 & \multirow{2}{*}{user-churn (3.9m)} & Test & \textbf{0.6988} & 0.694 & -0.69 \\
 & & Val & 0.7042 & 0.701 &  \\

\bottomrule
\end{tabular}
}
\end{minipage}
\hspace{2pt}
\begin{minipage}{.49\textwidth}
\centering
\small
\caption{Results on the entity regression tasks in RelBench. Lower is better. Best values are in \textbf{bold}. Relative gains are in percentage.}
\label{tab:main-results-classification}
\scalebox{0.63}{
\begin{tabular}{llccccc}
\toprule
\textbf{Dataset} & \textbf{Task (\# train)} & \textbf{MAE $\downarrow$} & \makecell{\textbf{RDL}\\\textbf{Baseline}} & \makecell{\textbf{Rel-GT}\\ \textbf{(ours)}} & \makecell{\textbf{Rel.}\\ \textbf{Gain}} \\
\midrule

\multirow{2}{*}{rel-f1} 
 & \multirow{2}{*}{driver-position (7k)} & Test & 4.022 & \textbf{3.917} & 2.61 \\
 & & Val & 3.193 & 3.326 & \\

\midrule
\multirow{2}{*}{rel-avito}
 & \multirow{2}{*}{ad-ctr (5k)} & Test & 0.041 & \textbf{0.035} & 14.63 \\
 & & Val & 0.037 & 0.031 & \\


\midrule
\multirow{2}{*}{rel-event}
 & \multirow{2}{*}{user-attendance (19k)} & Test & 0.258 & \textbf{0.250} & 3.10 \\
 & & Val & 0.255 & 0.255 & \\


\midrule
\multirow{4}{*}{rel-trial}
 & \multirow{2}{*}{study-adverse (43k)} & Test & 44.473 & \textbf{44.225} & 0.56 \\
 & & Val & 46.290 & 46.180 & \\
 & \multirow{2}{*}{site-success (151k)} & Test & 0.400 & \textbf{0.326} & 18.50 \\
 & & Val & 0.401 & 0.359 &  \\

\midrule
\multirow{4}{*}{rel-amazon}
 & \multirow{2}{*}{user-ltv (4.7m)} & Test & 14.313 & \textbf{14.266} & 0.33 \\
 & & Val & 12.132 & 12.115 & \\
 & \multirow{2}{*}{item-ltv (2.7m)} & Test & 50.053 & \textbf{48.670} & 2.76 \\
 & & Val & 45.1401 & 43.243 &  \\

\midrule
\multirow{2}{*}{rel-stack}
 & \multirow{2}{*}{post-votes (2.5m)} & Test & \textbf{0.065} & \textbf{0.065} & 0.00 \\
 & & Val & 0.059 & 0.059 & \\

\midrule
\multirow{2}{*}{rel-hm}
 & \multirow{2}{*}{item-sales (5.5m)} & Test & 0.056 & \textbf{0.053} & 5.36 \\
 & & Val & 0.065 & 0.062 & \\

\bottomrule
\end{tabular}
}
\end{minipage}
\end{table}





% Equations in section 3.1

% To process each token in the 5-tuple representation $(x_{v_j}, \phi(v_j), p(v_i, v_j), \tau(v_j) - \tau(v_i), \text{GNN-PE}_{v_j})$, we employ specialized encoders that transform each element into a $d$-dimensional vector space. The node feature encoding transforms the raw attributes using the PyTorch Frame encoder:
% \begin{equation}
%     \mathbf{h}_{\text{feat}}(v_j) = \text{Frame}(x_{v_j})
% \end{equation}

% For categorical elements, we use learnable embedding matrices. The node type encoding maps each table-specific entity type to a dense representation:
% \begin{equation}
%     \mathbf{h}_{\text{type}}(v_j) = \mathbf{W}_{\text{type}} \cdot \mathbf{onehot}(\phi(v_j))
% \end{equation}
% where $\mathbf{W}_{\text{type}} \in \mathbb{R}^{d \times |\mathcal{T}|}$ is the learnable weight matrix and $|\mathcal{T}|$ is the number of node types.

% Similarly, the hop distance encoding captures the structural proximity between nodes:
% \begin{equation}
%     \mathbf{h}_{\text{hop}}(v_i, v_j) = \mathbf{W}_{\text{hop}} \cdot \mathbf{onehot}(p(v_i, v_j))
% \end{equation}
% with $\mathbf{W}_{\text{hop}} \in \mathbb{R}^{d \times h_{\max}}$ mapping hop distances to vector representations.

% The temporal encoding linearly transforms the time difference between nodes:
% \begin{equation}
%     \mathbf{h}_{\text{time}}(v_i, v_j) = \mathbf{W}_{\text{time}} \cdot (\tau(v_j) - \tau(v_i)) + \mathbf{b}_{\text{time}}
% \end{equation}
% where $\mathbf{W}_{\text{time}} \in \mathbb{R}^{d \times 1}$ and $\mathbf{b}_{\text{time}} \in \mathbb{R}^{d}$ are learnable parameters.

% For capturing local graph structure, we apply a lightweight GNN to the subgraph:
% \begin{equation}
%     \mathbf{h}_{\text{pe}}(v_j) = \text{GNN}(\mathbf{A}_{\text{local}}, \mathbf{Z}_{\text{random}})_j
% \end{equation}
% where $\mathbf{A}_{\text{local}} \in \mathbb{R}^{K \times K}$ is the adjacency matrix of the sampled subgraph and $\mathbf{Z}_{\text{random}} \in \mathbb{R}^{K \times d_{\text{init}}}$ are randomly initialized node features.

% The final token representation combines all encoded elements:
% \begin{equation}
%     \mathbf{h}_{\text{token}}(v_j) = \mathbf{h}_{\text{feat}}(v_j) + \mathbf{h}_{\text{type}}(v_j) + \mathbf{h}_{\text{hop}}(v_i, v_j) + \mathbf{h}_{\text{time}}(v_i, v_j) + \mathbf{h}_{\text{pe}}(v_j)
% \end{equation}
